SSL^2: Self-Supervised Learning meets Semi-Supervised Learning: Multiple Sclerosis Segmentation in 7T-MRI from large-scale 3T-MRI

Automated segmentation of multiple sclerosis (MS) lesions from MRI scans is important to quantify disease progression. In recent years, convolutional neural networks (CNNs) have shown top performance for this task when a large amount of labeled data is available. However, the accuracy of CNNs suffers when dealing with few and/or sparsely labeled datasets. A potential solution is to leverage the information available in large public datasets in conjunction with a target dataset which only has limited labeled data. In this paper, we propose a training framework, SSL2 (self-supervised-semi-supervised), for multi-modality MS lesion segmentation with limited supervision. We adopt self-supervised learning to leverage the knowledge from large public 3T datasets to tackle the limitations of a small 7T target dataset. To leverage the information from unlabeled 7T data, we also evaluate state-of-the-art semi-supervised methods for other limited annotation settings, such as small labeled training size and sparse annotations. We use the shifted-window (Swin) transformer1 as our backbone network. The effectiveness of self-supervised and semi-supervised training strategies is evaluated in our in-house 7T MRI dataset. The results indicate that each strategy improves lesion segmentation for both limited training data size and for sparse labeling scenarios. The combined overall framework further improves the performance substantially compared to either of its components alone. Our proposed framework thus provides a promising solution for future data/label-hungry 7T MS studies.

==> review.tex <==
REVIEWER'S COMMENTS:

- The paper presents a new self-supervised learning method to segment multiple sclerosis (MS) lesions from 7T MRI images. Both public 3T and a partially labeled in house 7T datasets are used. The method is well justified and gives promising results. The paper needs a thorough grammar check.

- The authors proposed a Self-Supervised Semi-Supervised Learning (S4L) method to segment MS lesions on 7T MRI datasets while distilling knowledge from publicly available 3T datasets and some labeled 7T datasets. The idea is to use self-supervised training on 3T datasets by designing proxy tasks to minimize rotation prediction loss, inpainting reconstruction loss and contrastive loss from the input data and their augmented versions, while learning the encoder with Swin-Transformer.
The semi-supervised part leverages both labeled and unlabeled 7T data to fine tune the learning based on the trained Swin-transformer encoder. 8 semi-supervised methods were compared and the Mean Teacher and Cross Pseudo Supervision methods were the worst and best performing methods respectively.
Pros:
1) A very elaborate set of experiments were performed with almost all the publicly available datasets from brain lesion segmentation challenges, with 8 semi-supervised methods compared in different training paradigms.
2) The design of proxy task to learn the Swin-transformer encoder was innovative. Although it would be interesting to see if the encoder trained for a segmentation task performs differently.
Cons:
1) A small number of datasets were used to evaluate (n=14, 7T datasets) the methods.
2) The average Dice reported does not show the variance.
3) The typos and lack of punctuation marks should be corrected.
4) Details on the CPS and Mean teacher architectures must be presented in the camera-ready version.

- this manuscript presents a self- and semi- supervised training paradigm evaluated in a low sample context. The network itself included a SWIN Transformer encoder which is currently a very popular architecture giving good results in a variety of medical imaging tasks. A variety of strategies for training the network were used including pretraining of weights using a self-supervised task followed by task specific training. Task specific training was evaluated using a mean teacher and a cross pseudo-supervision (many other will be presented in the final manuscript).


The authors demonstrate their approach with the cross pseudo-supervision is able to give goo results for a MS lesion segmentation task even for very small numbers (>70\% for 5 samples). These are promising results for a very difficult and important problem in medical imaging and deep learning development on emerging technologies.

==> table3_backup.tex <==
\begin{table}[b]
    \centering
    \caption{Segmentation performance (Dice score) for 6 different semi-supervised models in our 7-fold cross-validation experiment (Sec.\ \ref{sec:semi-supervise}). The fully supervised model does not have access to any unlabeled samples and thus has the lowest performance. Bold indicates the best performance in each fold. Among the semi-supervised methods, Mean Teacher is the worst performer and Cross Pseudo Supervision is the top performer for the MS lesion segmentation task. }
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|l|l|l|l|l|l|l||l|l}
    \hline
        Methods & Fold 1 & Fold 2 & Fold 3 & Fold 4 & Fold 5 & Fold 6 & Fold 7 & Avg  & Std \\ \hline
        Fully Supervised\cite{zhang2019multiple} & 0.6982 & 0.6844 & 0.6867 & 0.6989 & 0.6744 & 0.6904 & 0.6964 & 0.6899 & 0.0089 \\ 
        Mean Teacher\cite{tarvainen2017mean} & 0.7107 & 0.7048 & 0.6991 & 0.7055 & 0.6990 & 0.7088 & 0.7048 & 0.7047 & 0.0044 \\ 
        Entropy Minimization\cite{vu2019advent} & 0.7238 & 0.7318 & 0.7312 & 0.7422 & 0.7320 & 0.7391 & 0.7257 & 0.7323 & 0.0066 \\
        Deep Adversarial Networks\cite{zhang2017deep} & 0.7283 & 0.7455 & 0.7294 & 0.7521 & 0.7252 & 0.7263 & 0.7241 & 0.7330 & 0.0111 \\ 
        Uncertainty Aware Mean Teacher \cite{yu2019uncertainty}& 0.7347 & 0.7246 & 0.7279 & 0.7351 & 0.7263 & 0.7352 & 0.7321 & 0.7308 & 0.0045 \\ 
        FixMatch\cite{sohn2020fixmatch, media2022urpc} & 0.7732 & 0.7753 & 0.7614 & \textbf{0.7897} & 0.7726 & 0.7656 & 0.7797 & 0.7739 & 0.0092 \\
        Cross Pseudo Supervision \cite{chen2021semi}& \textbf{0.7808} & \textbf{0.7894} & \textbf{0.7764} & 0.7834 & \textbf{0.7901} & \textbf{0.7803 }& \textbf{0.7844} & \textbf{0.7835} & 0.0050 \\ 
        \hline
    \end{tabular}
    }


        \label{tab:semi}

\end{table}

==> table_org.tex <==
\begin{table}[b]
\caption{Segmentation performance (Dice score) under varying amounts of training data availability. The central panel shows the results of the training data size experiment (Sec.~\ref{sec:training_variance}), whereas the right panel shows the sparse labeling experiment (Sec.~\ref{sec:sparse}). }
\label{tab:archive}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l"lll"llll|}
\hline
\multirow{2}{*}{Methods} &
  \multicolumn{3}{c"}{Training data size experiment} &
  \multicolumn{4}{c|}{Sparse or uncertain labeling experiment} \\ \cline{2-8} 
 &
  \multicolumn{1}{l|}{3 training samples} &
  \multicolumn{1}{l|}{5 training samples} &
  10 training samples &
  \multicolumn{1}{l|}{10\%} &
  \multicolumn{1}{l|}{20\%} &
  \multicolumn{1}{l|}{50\%} &
  100\% \\ \hline
Training from scratch &
  \multicolumn{1}{l|}{0.5232} &
  \multicolumn{1}{l|}{0.6233} &
  0.6727 &
  \multicolumn{1}{l|}{0.5174} &
  \multicolumn{1}{l|}{0.5732} &
  \multicolumn{1}{l|}{0.6542} &
  0.6971 \\ \hline
Training with self-supervised pre-training &
  \multicolumn{1}{l|}{0.5328} &
  \multicolumn{1}{l|}{0.6158} &
  0.6971 &
  \multicolumn{1}{l|}{0.6233} &
  \multicolumn{1}{l|}{0.6422} &
  \multicolumn{1}{l|}{0.6855} &
  0.7121 \\ \hline
Mean-Teacher &
  \multicolumn{1}{l|}{0.5727} &
  \multicolumn{1}{l|}{0.6523} &
  0.7024 &
  \multicolumn{1}{l|}{0.5673} &
  \multicolumn{1}{l|}{0.5884} &
  \multicolumn{1}{l|}{0.6627} &
  0.7047 \\ \hline
Cross pseudo Supervision &
  \multicolumn{1}{l|}{0.6272} &
  \multicolumn{1}{l|}{0.6942} &
  0.7699 &
  \multicolumn{1}{l|}{0.6107} &
  \multicolumn{1}{l|}{0.6342} &
  \multicolumn{1}{l|}{0.7108} &
  0.7835 \\ \hline
Mean-Teacher + Self-supervised &
  \multicolumn{1}{l|}{0.6384} &
  \multicolumn{1}{l|}{0.6722} &
  0.7058 &
  \multicolumn{1}{l|}{0.6411} &
  \multicolumn{1}{l|}{0.6589} &
  \multicolumn{1}{l|}{0.7232} &
  0.7624 \\ \hline
Cross pseudo Supervision + Self-supervised &
  \multicolumn{1}{l|}{\textbf{0.6485}} &
  \multicolumn{1}{l|}{\textbf{0.7325}} &
  \textbf{0.7884} &
  \multicolumn{1}{l|}{\textbf{0.6523}} &
  \multicolumn{1}{l|}{\textbf{0.6785}} &
  \multicolumn{1}{l|}{\textbf{0.7823}} &
  \textbf{0.8186} \\ \hline
\end{tabular}
}
\end{table}
